Spectra and pseudo-spectra of tridiagonal $k$-Toeplitz matrices and the topological origin of the non-Hermitian skin effect

We establish new results on the spectra and pseudo-spectra of tridiagonal $k$-Toeplitz operators and matrices. In particular, we prove the connection between the winding number of the eigenvalues of the symbol function and the exponential decay of the associated eigenvectors (or pseudo-eigenvectors). Our results elucidate the topological origin of the non-Hermitian skin effect in general one-dimensional polymer systems of subwavelength resonators with imaginary gauge potentials, proving the observation and conjecture in arXiv:2307.13551. We also numerically verify our theory for these systems.

==> Ideas.tex <==




\textbf{New idea:} 
    When $z_1=z_2$ for $\lambda_0$, we define for $s\geq 2$
    \[
    Q(z) := z^s\det(f(z)-\lambda_0) = (z-z_1)^2P(\lambda_0)z^{s-1},
    \]
    which gives 
    \[
    Q'(z) = 2(z-z_1)P(\lambda_0)z^{s-1}+ (z-z_1)^2P(\lambda_0)(s-1)z^{s-2}.
    \]
    On the other hand, by
    \[
    z^s\det(f(z)-\lambda_0) = Az^{s+1} + Bz^{s-1} + g(\lambda_0)z^s,
    \]
   we have 
   \[
   Q'(z) = (s+1)z^{s}A+ (s-1)z^{s-2}B+ sz^{s-1}g(\lambda). 
   \]
   Check if this $\frac{Q'(z)}{z^{s-1}}$ is actually \todo[color = yellow]{Then here we would have to adjust to $\det(f_1(z)-\frac{1}{s}\lambda)$ }
   \[
\det(f_1(z)-\lambda)
   \]
    where 
    \[
  f_1(z) = (s-1)z^{-1}S+ sD + (s+1)zE.
  % \begin{pmatrix}
  %       a_1 & b_1 & 0 & \dots & 0 & ()c_kz^{-1} \\
  %       c_2 & a_2 & b_2 & 0 & \dots & 0 \\
  %       0 & c_3 & a_3 & b_3 & \ddots & \vdots \\
  %       \vdots  & \ddots &  \ddots & \ddots & \ddots & 0 \\
  %       0 & \dots & 0 & c_{k-1} & a_{k-1}& b_{k-1}\\
  %       b_kz & 0 &  \dots & 0 & c_k & a_k \\       
  %   \end{pmatrix}.
    \]

\textbf{An attempt to show it:} using Lemma\ref{lem:tridiagonaldeterminant}
\begin{equation*}
    \operatorname{det}(f_1(z)-\lambda) = (-1)^{k+1}s^{k-1}(s-1) (\prod_{i=1}^k c_i)z^{-1} + (-1)^{k+1}s^{k-1}(s+1)(\prod_{i=1}^kb_i)z + \Tilde{g}(\lambda)
\end{equation*}
using the expansion of $\Tilde{g}(\lambda)$ taking into account the form of the symbol $f_1(z)$.\todo[color = yellow]{Assuming the small correction fo the previous lemma}
\begin{align*}
    \Tilde{g}(\lambda) &= \begin{vmatrix}
            s(a_1 - \frac{1}{s}\lambda) & sb_1 & 0 & \dots & 0 \\
            sc_1 & s(a_2 - \frac{1}{s}\lambda) & sb_2 & \ddots & \vdots \\
            0 & \ddots & \ddots & \ddots & 0 \\
            \vdots & \ddots & \ddots & \ddots & sb_{k-1} \\
            0 & \dots & 0 & sc_{k-1} & s(a_{k} - \frac{1}{s}\lambda) \\
        \end{vmatrix} \\
        &- (s+1)b_k(s-1)c_1\begin{vmatrix}
            s(a_2 - \frac{1}{s}\lambda) & sb_2 & 0 & \dots & 0 \\
            sc_3 & s(a_3 - \frac{1}{s}\lambda) & sb_3 & \ddots & \vdots \\
            0 & \ddots & \ddots & \ddots & 0 \\
            \vdots & \ddots & \ddots & \ddots & sb_{k-2} \\
            0 & \dots & 0 & sc_{k-1} & s(a_{k-1} - \frac{1}{s}\lambda) \\
        \end{vmatrix}\\
        &=s^k \begin{vmatrix}
            a_1 - \frac{1}{s}\lambda & b_1 & 0 & \dots & 0 \\
            c_1 & a_2 - \frac{1}{s}\lambda & b_2 & \ddots & \vdots \\
            0 & \ddots & \ddots & \ddots & 0 \\
            \vdots & \ddots & \ddots & \ddots & b_{k-1} \\
            0 & \dots & 0 & c_{k-1} & a_{k} - \frac{1}{s}\lambda \\
        \end{vmatrix} \\
        &-(s^2-1) b_k  c_1 s^{k-2} \begin{vmatrix}
            a_2 - \frac{1}{s}\lambda & b_2 & 0 & \dots & 0 \\
            c_3 & a_3 -\frac{1}{s}\lambda & sb_3 & \ddots & \vdots \\
            0 & \ddots & \ddots & \ddots & 0 \\
            \vdots & \ddots & \ddots & \ddots & b_{k-2} \\
            0 & \dots & 0 & c_{k-1} & a_{k-1} - \frac{1}{s}\lambda \\
        \end{vmatrix}\\
        &=s^kg(\frac{\lambda}{s})+b_k c_1 s^{k-2} 
        \begin{vmatrix}
            a_2 - \frac{1}{s}\lambda & b_2 & 0 & \dots & 0 \\
            c_3 & a_3 -\frac{1}{s}\lambda & sb_3 & \ddots & \vdots \\
            0 & \ddots & \ddots & \ddots & 0 \\
            \vdots & \ddots & \ddots & \ddots & b_{k-2} \\
            0 & \dots & 0 & c_{k-1} & a_{k-1} - \frac{1}{s}\lambda \\
        \end{vmatrix}\\
\end{align*}
Hence, unfortunately
\begin{equation*}
    s^{k-1}z^{1-s}Q'(z) = \det(f_1(z)-s\lambda_0) - b_k c_1 s^{k-2} 
        \begin{vmatrix}
            a_2 - \lambda_0 & b_2 & 0 & \dots & 0 \\
            c_3 & a_3 -\lambda_0 & sb_3 & \ddots & \vdots \\
            0 & \ddots & \ddots & \ddots & 0 \\
            \vdots & \ddots & \ddots & \ddots & b_{k-2} \\
            0 & \dots & 0 & c_{k-1} & a_{k-1} - \lambda_0 \\
        \end{vmatrix}\\
\end{equation*}
\todo[color = yellow]{Could this be correct?}
\todo[color=cyan]{There was a mistake in the initial computation.}







As $ker(f(z_0)-\lambda_0)$ is dimension one, as the construction is trivial when $ker(f(z_0)-\lambda_0)\geqslant 2$. Now consider the decomposition of $\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)$ in $ker(f(z_0)-\lambda_0)$ and $ker(f(z_0)-\lambda_0)^{\perp}$. Denote 
\[
P_{ker(f(z_0)-\lambda_0)^{\perp}}(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))
\]
as the projection of $(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))$ onto space $ker(f(z_0)-\lambda_0)^{\perp}$. It is not hard to see that its norm is non-zero and should also be bounded below by a positive constant. From (\ref{equ:proofexpoentialdecay3}) we have 
\begin{equation}\label{equ:proofexpoentialdecay2}
\begin{aligned}
&(S+ (D-\lambda(\epsilon_j))z_1(\epsilon_j)+E z_1(\epsilon_j)^2)\frac{P_{ker(f(z_0)-\lambda_0)^{\perp}}(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta(\epsilon_j)}\\
=&- \left((D-\lambda(\epsilon_j))\frac{(z_1(\epsilon_j)-z_2(\epsilon_j))\vect w_2(\epsilon_j))}{\Delta(\epsilon_j)}+E \frac{(z_1(\epsilon_j)^2-z_2(\epsilon_j)^2)\vect w_2(\epsilon_j)}{\Delta(\epsilon_j)}\right)\\
& -(S+ (D-\lambda(\epsilon_j))z_1(\epsilon_j)+E z_1(\epsilon_j)^2)\frac{P_{ker(f(z_0)-\lambda_0)}(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta(\epsilon_j)}.
\end{aligned}
\end{equation}
Since the norm of RHS of above equation is bounded below and above by positive constants. 
{\color{red} The second term of the RHS seems could blow up. We now need to prove that the order of $(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))$ is of or smaller than $O(\Delta(\epsilon_j))$ which should be possible to be solved now. It is possible that there is no limit of $\frac{(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta(\epsilon_j)}$, thus estimating the order of $\frac{(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta(\epsilon_j)}$  seems inevitable. }\\
{\color{blue} By a numerical computation we should expect $\mathcal{O}(\sqrt{\Delta(\epsilon_j)})$}
{\color{red} $\Delta(\epsilon_j)$ is $z_1-z_2$, it is $O(\sqrt{\epsilon})$}

\textbf{Asymptotics:} One can easily show via the discriminant that $\mathcal{O}(\Delta(z)) = \mathcal{O}(\sqrt{\Delta(\epsilon)})$. It remains to show that $(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))$ has order $\mathcal{O}(\Delta z)$. Therefore, we could solve the eigenvalue problem explicitly. This wields a system of equations 
\begin{equation}
    \begin{cases}
        a_1 w_1 + b_1 w_2 + w_k c_k z^{-1} = \lambda w_1 \\
        c_j w_j + a_{j+1}w_{j+1} + b_{j+1} w_{j+2} = \lambda w_{j+1} \\
        w_1 b_k z + c_{k-1}w_{k-1} + a_k w_k = \lambda w_k
    \end{cases}
\end{equation}



WLOG we assume that the first entry is $w_k = 1$, otherwise one could always scale the entire vector by a scalar. Furthermore, we are only interested in the asymptotics of the vector so we don't have to explicitly compute each vector entry. The first equation then yields:

This now is enough to prove that there exists a subsequence $\hat \epsilon_j$ of $\epsilon_j$'s so that 
\[
\lim_{\hat \epsilon_j\rightarrow 0}\frac{P_{ker(f(z_0)-\lambda_0)^{\perp}}(\vect w_1(\hat \epsilon_j)-\vect w_2(\hat \epsilon_j))}{\Delta(\hat \epsilon_j)} = \vect v_1
\]
for some $\vect v_1\in \mathbb R^{k}$. By (\ref{equ:proofexpoentialdecay2}), this gives 
\[
(S+ (D-\lambda_0)z_0+E z_0^2)\vect v_1 = -((D-\lambda_0)+2z_0E)\vect v_0. 
\]
This justifies the existence of the $\vect v_1$. Combined with previous arguments, $\vect u_2$ is a desired construction vector. 


%The existence can be derived from considering several cases. \\
% \todo[color = yellow]{I heavily abused the notation for vectors here. We'll have to come up with a more clean way.}

% \textbf{Idea:} We show that a from $\mathbf{v_0}$ linearly independent $\mathbf{v_1}$ exists and then argue that a linear combination of both is if the from $\mathbf{u_2}$.\\
% Now we show the existence of such a vector $\mathbf{v_1}$ by giving its explicit construction.
% Suppose we have a double root $z_0$ for $\lambda_0$. Thus, $z_1, z_2 \xrightarrow{\lambda_1, \lambda_2 \to \lambda_0}z_0$. 
% As we are taking the limit we can assume that for $z_1$ and $z_2$ exist corresponding eigenvectors $\mathbf{v_1}$ and $\mathbf{v_2}$ such that $f(z_1)\mathbf{v_1} = \lambda_1 \mathbf{v_1}$ and $f(z_2)\mathbf{v_2} = \lambda_2 \mathbf{v_2}$. The limit vector as $z_1, z_2 \to z_0$ is of the form
% \begin{equation}
% \mathbf{v_0} = (\mathbf{v_1} - \mathbf{v_2}, z_1 \mathbf{v_1} - z_2\mathbf{v_2}, \cdots )
% \end{equation}
% We denote the entries of the vector $\mathbf{v_0}$ by $z_1^j\mathbf{v_1}- z_2^j\mathbf{v_2}$, where $j = 0, 1, \cdots, k$.
% To show that the entries of $\mathbf{v_0}$ are not zero, consider the scalation by $\frac{1}{\Delta z}$, where $\Delta z = z_2-z_1$. For the vector entries, we then get
% \begin{align*}
%     \frac{z_1^j\mathbf{v_1}- z_2^j\mathbf{v_2}}{\Delta z} &= \frac{z_1^j\mathbf{v_1}-z_1^j \mathbf{v_2} + z_1^j \mathbf{v_2} -z_2^j\mathbf{v_2}}{\Delta z}\\
%     &= z_1^j\frac{\mathbf{v_1}-\mathbf{v_2}}{\Delta z} + \mathbf{v_2} \frac{z_1^j-z_2^j}{\Delta z}
% \end{align*}

% Note that the second term contains the derivative of the function $f(z) = z^j$, i.e. $f'(z) = jz^{j-1}$. We now show that  $\frac{\mathbf{v_1}-\mathbf{v_2}}{\Delta z} = \mathbf{C}$
% %begin{equation*}
% %    Az^2 + B + g(\lambda + \varepsilon)z = 0 \quad \text{as } \varepsilon \to 0.
% %%As $g(\lambda)$ is a polynomial of degree $k$ we may write
% %\begin{equation*}
% %    Az^2 + B + (g(\lambda) + \mathcal{O}(\varepsilon))z = 0 \quad \text{as } \varepsilon \to 0.
% %\end{equation*}
% %Computing the discriminant roots we obtain
% %\begin{equation*}
% %    z_{1,2} = \frac{-(g(\lambda) + \mathcal{O}(\varepsilon)) \pm \sqrt{ (g(\lambda) + \mathcal{O}(\varepsilon))^2 - 4AB}}{2A}
% %\end{equation*}
% %\begin{equation*}
% %    \Delta z = \mathcal{O}(\sqrt{\varepsilon}) \quad \text{as } \varepsilon \to 0.
% %\end{equation*}
% , i.e. show that the derivative of the vectors is a constant not equal to $0$ in $z_0$.
% Therefore we first recall a known result from \cite[Theorem 8, p.130]{lax07}
% \begin{theorem}\label{thm: existence of eigenvector}
%      Let $A(t)$ be a differentiable matrix-valued function of $t$, $a(t)$ an eigenvalue of $A(t)$ of multiplicity one. Then we can choose an eigenvector $h(t)$ of $A(t)$ pertaining to the eigenvalue $a(t)$ to depend differentiably on $t$.
% \end{theorem}
% First note that $z_1, z_2 \xrightarrow{\lambda \to \lambda_0}z_0 \in \R$ so one can chose $z_1, z_2 \in \R$. In our case, the matrix-valued function is our symbol function $f(z)$ which is differentiable and continuous. Furthermore, $f(z)$ has two eigenvalues of multiplicity $1$ at $z_1$ and $z_2$. Then, by Theorem\ref{thm: existence of eigenvector} we may find an eigenvector $\mathbf{v_0}(z)$ that depends on $z$ and is differentiable. In other words, the eigenvector is continuous w.r.t. to the symbol function $f(z)$ and its derivative exists.
% All that remains is to show that the 'derivative' of the vector is nonzero in $z_0$. Suppose for contradiction that $\frac{d }{dz}\mathbf{v_i}(z_0) = 0,  \forall i$. Then we get from the eigenvalue problem the following system
% \begin{equation*}
%     f(z) \mathbf{v} = \lambda \mathbf{v} \quad z = z_1, z_2 \quad\mathbf{v}\neq 0
% \end{equation*}
% or explicitly
% \begin{equation*}
%     \begin{pmatrix}
%         a_1 & b_1 & 0 & \dots & 0 & c_k z^{-1} \\
%         c_1 & a_2 & b_2 & 0 & \dots & 0 \\
%         0 & c_2 & a_3 & b_3 & \ddots & \vdots \\
%         \vdots  & \ddots &  \ddots & \ddots & \ddots & 0 \\
%         0 & \dots & 0 & c_{k-2} & a_{k-1}& b_{k-1}\\
%         b_kz & 0 &  \dots & 0 & c_{k-1} & a_k \\       
%     \end{pmatrix} \begin{pmatrix}
%         \mathbf{v_1} \\
%         \mathbf{v_2} \\
%         \vdots\\
%         \vdots\\
%         \mathbf{v_{k-1}}\\
%         \mathbf{v_k}
%     \end{pmatrix} = \lambda \begin{pmatrix}
%         \mathbf{v_1} \\
%         \mathbf{v_2} \\
%         \vdots\\
%         \vdots\\
%         \mathbf{v_{k-1}}\\
%         \mathbf{v_k}
%     \end{pmatrix}
% \end{equation*}
% in other words, we obtain a system of linear equations that looks as follows
% \begin{equation*}
%     \begin{cases}
%         (a_1- \lambda) \mathbf{v_1}(z) + b_1 \mathbf{v_2}(z)  + c_k \frac{1}{z}\mathbf{v_k}(z)= 0 \label{eq: system 1} \\
%         c_j \mathbf{v_j}(z) + (a_{j+1}-\lambda)\mathbf{v_{j+1}}(z) + b_{j+1} \mathbf{v_{j+2}}(z)=0 \quad j = \{ 1, ... , k-2\}\\
%         b_k z \mathbf{v_1}(z) + c_{k-1}\mathbf{v_{k-1}}(z) + (a_k-\lambda) \mathbf{v_k}(z) = 0
%     \end{cases}
% \end{equation*}
% consider the first equation  and differentiate w.r.t. $z$, then
% \begin{equation*}
%     (a_1- \lambda) \underbrace{\mathbf{v_1}'(z_0)}_{=0} + b_1 \underbrace{\mathbf{v_2}'(z_0)}_{=0}  + c_k \frac{1}{z_0}\underbrace{\mathbf{v_k}'(z_0)}_{=0}-\frac{1}{z_0^2}\mathbf{v_k}(z_0) = 0 
% \end{equation*}
% which then implies that $\mathbf{v_k}(z_0) = 0$.
% By a similar argument applied to the last eigenvector entry yields
% \begin{equation}
%     \mathbf{v_k}(z_0) = 0
% \end{equation}
% knowing that $\mathbf{v_1}(z_0) = \mathbf{v_k}(z_0) = 0$ we find by the first equation that $\mathbf{v_2}(z_0) = 0$ and by all the other equations one can easily verify that $\mathbf{v_i}(z_0) = 0, \forall i$. But we know by assumption that $\mathbf{v}$ is a true eigenvector not equal to $0$. So we get a contradiction and conclude
% \begin{equation}
%     \frac{\mathbf{v_1}-\mathbf{v_2}}{\Delta z} = \Vec{C} \neq \Vec{0}.
% \end{equation}
% Indeed this limit exists and is finite. Then our vector $\mathbf{v}$ looks as follows
% \begin{equation*}
%      \mathbf{v}_j = z^j\mathbf{C}  + jz^{j-1}\mathbf{v}_1 \quad j =1,..., k
% \end{equation*}
% in other words, suppose that we  have found the vector $\mathbf{v_0}$ then one can construct a linearly independent vector $\mathbf{v_1}$ which is of the form
% \begin{equation*}
%     \mathbf{v_1} = \frac{d}{dz}\mathbf{v_0}(z)|_{z = z_0}
% \end{equation*}
% which concludes the existence of such a $v_1$ and also the vector $\mathbf{u_2}$ is of the correct form.
%\end{proof}


For $\mathbf{u_i}$ to be an eigenvector, for $j \geq m$ we find the condition.  
    \begin{align*}
        &S(z^j_0\mathbf{v_1} + (z_0^{j})^{(m)}\mathbf{v_0}) + (D-\lambda_0) (z_0^{j+1} \mathbf{v_1} + (z_0^{j+1})^{(m)}\mathbf{v_0}) + E(z_0^{j+2}\mathbf{v_1} + (z_0^{j+2})^{(m)}\mathbf{v_0})\\
        &= z_0^j\left(S(\mathbf{v_1} + j\cdot...\cdot (j-m+1)z_0^{-m}\mathbf{v_0}) + (D-\lambda_0)(z_0\mathbf{v_1} + (j+1)\cdot...\cdot (j-m+2)z_0^{-m+1}\mathbf{v_0})\right.\\
        &\qquad \quad\left.+ E(z_0^2\mathbf{v_1} + (j+2)\cdot...\cdot (j-m+3)z_0^{-m+2}\mathbf{v_0})\right)\\
        &= z_0^j\left((S+ (D-\lambda_0)z_0 + Ez_0^2)\mathbf{v_1} +(S\cdot j\cdot...\cdot(j-m+1)z_0^{-m}\right.\\
        &\quad \left.+ (D-\lambda_0)\cdot (j+1)\cdot...\cdot (j-m+2)z_0^{-m+1}) + E\cdot (j+2)\cdot...\cdot (j-m+3)z_0^{-m+2})\mathbf{v_0}\right)\\
        &= z_0^j\left((S+ (D-\lambda_0)z_0 + Ez_0^2)\mathbf{v_1} + z_0^{-m}(S\cdot j\cdot...\cdot(j-m+1)\right.\\
        &\quad \left.+ (D-\lambda_0)\cdot (j+1)\cdot...\cdot (j-m+2)z_0^{+1}) + E\cdot (j+2)\cdot...\cdot (j-m+3)z_0^{2})\mathbf{v_0}\right)
    \end{align*}
    Thus for $\mathbf{u_i}$ to be an eigenvector, we only need \todo[color = yellow]{By the fact that $\mathbf{v_1}$ is an eigenvector one can further simplify this, in particular the first term can be killed.}
    \begin{multline}\label{eq: condition_block_eigenvector}
        (S+ (D-\lambda_0)z_0 + Ez_0^2)\mathbf{v_1} =-\left(S\cdot j\cdot...\cdot(j-m+1)z_0^{-m}\right. \\ \quad \left.+ (D-\lambda_0)\cdot (j+1)\cdot...\cdot (j-m+2)z_0^{-m+1})+ E\cdot (j+2)\cdot...\cdot (j-m+3)z_0^{-m+2}\right)\mathbf{v_0}
    \end{multline}
    \todo[color=cyan]{I am pretty sure that this is not the right condition}
    \todo[color = yellow]{indeed we should use the Laplace formula here.}


    \begin{equation}\label{equ:proof_band_expoentialdecay}
\begin{aligned}
&S\frac{\vect w_a^{(m-1)}(\epsilon_j)-\vect w_b^{(m-1)}(\epsilon_j)}{\Delta(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_a(\epsilon_j)\vect w_a^{(m-1)}(\epsilon_j)-z_b(\epsilon_j)\vect w_b^{(m-1)}(\epsilon_j)}{\Delta(\epsilon_j)}\\
& \qquad +E\frac{z_a(\epsilon_j)^2\vect w_a^{(m-1)}(\epsilon_j)-z_b(\epsilon_j)^2\vect w_b^{(m-1)}(\epsilon_j)}{\Delta(\epsilon_j)} =0
\end{aligned}
\end{equation}
where $\Delta(\epsilon_j):=z_a(\epsilon_j)-z_b(\epsilon_j)$ and 
\begin{equation}\label{equ:proof_band_expoentialdecay}
\begin{aligned}
&S\frac{\vect w_a^{(m-1)}(\epsilon_j)-\vect w_b^{(m-1)}(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_a(\epsilon_j)\vect w_a^{(m-1)}(\epsilon_j)-z_b(\epsilon_j)\vect w_b^{(m-1)}(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}\\
& \qquad +E\frac{z_a(\epsilon_j)^2\vect w_a^{(m-1)}(\epsilon_j)-z_b(\epsilon_j)^2\vect w_b^{(m-1)}(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)} =0
\end{aligned}
\end{equation}
where $\Delta_{\vect w}(\epsilon_j):= \bnorm{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}_2$.
This can alternatively be expressed as \todo[color = yellow]{Needs fixing. Needs the right condition.}

\begin{equation}\label{equ:proof_band_expoentialdecay}
\begin{aligned}
&S\frac{\vect w_a^{(m-1)}(\epsilon_j)-\vect w_b^{(m-1)}(\epsilon_j)}{\Delta(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_a(\epsilon_j)(\vect w_a^{(m-1)}(\epsilon_j)-\vect w_b^{(m-1)}(\epsilon_j))}{\Delta(\epsilon_j)}\\
&\qquad\qquad+E \frac{z_a(\epsilon_j)^2(\vect w_a^{(m-1)}(\epsilon_j)-\vect w_b^{(m-1)}(\epsilon_j))}{\Delta(\epsilon_j)}\\
=&- \left((D-\lambda(\epsilon_j))\frac{(z_a(\epsilon_j)-z_b(\epsilon_j))}{\Delta(\epsilon_j)}\vect w_b^{(m-1)}(\epsilon_j)+E \frac{(z_a(\epsilon_j)^2)-(z_b(\epsilon_j)^2)}{\Delta(\epsilon_j)}\vect w_b^{(m-1)}(\epsilon_j)\right).
\end{aligned}
\end{equation}
Note that $z_a$ and $z_b$ have been derived in previous computations and consist of the $(m-1)$-th derivative of $z^j$.
If there exists a subsequence $\hat \epsilon_j$'s of $\epsilon_j$'s so that the norm of $\frac{\vect w_a^{(m-1)}(\hat \epsilon_j)-\vect w_b^{(m-1)}(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}$ is bounded, considering a subsequence of $\hat \epsilon_j$'s is enough to prove the existence of the limit and hence prove the existence of such $\vect v_1$ so that 


\todo[color = yellow]{Use the right expression here.}
\begin{equation}\label{equ:proof_band_expoentialdecay13}
\left(S+(D-\lambda_0)z_0+Ez_0^{2}\right) \mathbf{v_1} = -\left((D-\lambda_0)+2z_0E\right) \mathbf{v_0}.
\end{equation}
Suppose now that there is no subsequence $\hat \epsilon_j$'s of $\epsilon_j$'s so that the norm of $\frac{\vect w_a^{(m-1)}(\hat \epsilon_j)-\vect w_b^{(m-1)}(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}$ is bounded. Thus there exists a subsequence $\hat \epsilon_j$'s of $\epsilon_j$'s so that the norm of $\frac{\vect w_a^{(m-1)}(\hat \epsilon_j)-\vect w_b^{(m-1)}(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}$ tends to infinity. This is 
\[
\babs{\frac{\Delta_{\vect w}(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}}\rightarrow +\infty, 
\]
which gives 
\begin{equation}\label{equ:proof_band_expoentialdecay8}
\babs{\frac{\Delta(\hat \epsilon_j)}{\Delta_{\vect w}(\hat \epsilon_j)}}\rightarrow 0. 
\end{equation}
On the other hand, (\ref{equ:proof_band_expoentialdecay5}) gives
\begin{equation}\label{equ:proof_band_expoentialdecay7}
\begin{aligned}
&S\frac{\vect w_a^{(m-1)}(\epsilon_j)-\vect w_b^{(m-1)}(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_a(\epsilon_j)(\vect w_a^{(m-1)}(\epsilon_j)-\vect w_b^{(m-1)}(\epsilon_j))}{\Delta_{\vect w}(\epsilon_j)}\\
&\qquad\qquad +E \frac{z_a(\epsilon_j)^2(\vect w_a^{(m-1)}(\epsilon_j)-\vect w_b^{(m-1)}(\epsilon_j))}{\Delta_{\vect w}(\epsilon_j)}\\
=&- \left((D-\lambda(\epsilon_j))\frac{(z_a(\epsilon_j)-z_b(\epsilon_j))\vect w_b^{(m-1)}(\epsilon_j))}{\Delta_{\vect w}(\epsilon_j)}+E \frac{(z_1(\epsilon_j)^2-z_b(\epsilon_j)^2)\vect w_b^{(m-1)}(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}\right).
\end{aligned}
\end{equation}
Then (\ref{equ:proof_band_expoentialdecay8}) indicates that there exists a subsequence $\tilde \epsilon_j$'s of $\hat \epsilon_j$'s so that 
\[
\lim_{\tilde \epsilon_j\rightarrow 0} (S+(D-\lambda(\tilde \epsilon_j))z_0 + 2z_0^2E)\frac{\vect w_a^{(m-1)}(\tilde\epsilon_j)-\vect w_b^{(m-1)}(\tilde\epsilon_j)}{\Delta_{\vect w}(\tilde\epsilon_j)} = \vect 0.
\]
Note that the boundedness of $\frac{\vect w_a^{(m-1)}(\tilde\epsilon_j)-\vect w_b^{(m-1)}(\tilde\epsilon_j)}{\Delta_{\vect w}(\tilde\epsilon_j)}$ is also important for deriving the above limit. This gives 
\begin{equation}\label{equ:proof_band_expoentialdecay12}
(S+(D-\lambda_0)z_0 + 2z_0^2E)\vect v_1 = \vect 0,
\end{equation}
for a certain vector $\vect v_1$ with $\bnorm{\vect v_1}_2=1$. Now we prove that $\vect v_1\neq \vect v_0$ and $\vect v_1 \neq -\vect v_0$. As $\vect v_1$ is the limit of 
\[
\frac{\vect w_a^{(m-1)}(\tilde\epsilon_j)-\vect w_b^{(m-1)}(\tilde\epsilon_j)}{\Delta_{\vect w}(\tilde\epsilon_j)},
\]
a key observation is that, since (\ref{equ:proof_band_expoentialdecay}) and (\ref{equ:proof_band_expoentialdecay10}), the angle between 
$\vect w_a^{(m-1)}(\tilde\epsilon_j)-\vect w_b^{(m-1)}(\tilde\epsilon_j)$ and $\vect v_0$ should approximate $\frac{\pi}{2}$. This is enough to demonstrate $\vect v_1\neq \vect v_0$ and $\vect v_1 \neq -\vect v_0$. Now, (\ref{equ:proof_band_expoentialdecay12}) contradicts the condition that $\vect v_0$ is the only eigenvector of $f(z_0)$ corresponding to the eigenvalue $\lambda_0$. Thus this case does not hold, we only have the case that $\frac{\vect w_a^{(m-1)}(\tilde\epsilon_j)-\vect w_b^{(m-1)}(\tilde\epsilon_j)}{\Delta_{\vect w}(\tilde\epsilon_j)}$ are uniformly bound. Then (\ref{equ:proof_band_expoentialdecay13}) already demonstrates the existence. This completes the proof. 


\textbf{WIP:}
    For $m \geq 3$ we may rewrite the second term, taking into account that $\mathbf{v_0}$ is an eigenvalue of $f(z)$\todo[color = yellow]{To get this simplification we need to have $m \geq 3$. in order to get overlap and ability to factor.}
    \begin{align*}
       &j\cdot...\cdot(j-m+3) \left( S(j-m+2)(j-m+1) z_0^{-m} + (D-\lambda_0) \cdot (j+1)(j-m+2) z_0^{-m+1}\right. \\
        &\qquad \left. + E \cdot(j+2)(j+1) z_0^{-m+2} \right)\\
        &=j\cdot...\cdot(j-m+3) z_0^{-m}\left( S(-2jm + m^2 -3m) + (D-\lambda_0) \cdot (-jm -m) z_0\right)
    \end{align*}
    Thus we only need
    \begin{equation*}
        \left(S+(D-\lambda_0)z_0+Ez_0^{2}\right) \mathbf{v_1} = j\cdot...\cdot(j-m+3) z_0^{-m}S(-2jm + m^2 -3m) + (D-\lambda_0) \cdot (-jm -m) z_0
    \end{equation*}



For $\mathbf{u_i}$ to be an eigentor we find the condition.
\begin{equation}\label{eq: condition_l_block}
    S\left(\mathbf{v_1} z_0^j + (z_0^j\mathbf{v_0})^{(n)}\right) + (D-\lambda_0)\left(\mathbf{v_1}z_0^{j+1} + (\mathbf{v_0}z_0^{j+1})^{(n)}\right)  + E\left( \mathbf{v_1} z_0^{j+2} + (\mathbf{v_0}z_0^{j+2})^{(n)}\right)
\end{equation}
This can be further simplified using the Leibnitz formula for products
\begin{align}
    (z_0^j\mathbf{v_0})^{(n)} &= \sum_{l = 0}^{n}\binom{n}{l}\vect (z_0^j)^{(l)}\vect v_0^{(n-l)}\mathds{1}_{j > l} \\
    &=  \sum_{l = 0}^{n}\binom{n}{l} \frac{j!}{(j-l)!}z_0^{j-l}\vect v_0^{(n-l)}\mathds{1}_{j > l}\\
    &= z_0^j \sum_{l = 0}^{n}\binom{n}{l} \frac{j!}{(j-l)!}z_0^{-l}\vect v_0^{(n-l)}\mathds{1}_{j > l}
\end{align}
The expressions for $(\mathbf{v_0}z_0^{j+1})^{(n)}$, $(\mathbf{v_0}z_0^{j+2})^{(n)}$, can by a similar procedure. That way (\ref{eq: condition_l_block}) simplifies to for $j \geq n$
\begin{align*}
    &z_0^{j} \left(S\left(\mathbf{v_1} + \sum_{l = 0}^{n}\binom{n}{l} \frac{j!}{(j-l)!}z_0^{-l}\vect v_0^{(n-l)}\right) + (D-\lambda) \left(\mathbf{v_1}z_0 + \sum_{l = 0}^{n}\binom{n}{l} \frac{(j+1)!}{(j+1-l)!}z_0^{1-l}\vect v_0^{(n-l)}\right)\right.  \\
    &\qquad\qquad\qquad\qquad\qquad\qquad \qquad +\left.E\left( \mathbf{v_1}z_0^2 + \sum_{l = 0}^{n}\binom{n}{l} \frac{(j+2)!}{(j+2-l)!}z_0^{2-l}\vect v_0^{(n-l)}\right)\right)\\
    %&=z_0^j\left(\left(S + (D-\lambda_0)z_0 + Ez_0^2\right)\mathbf{v_1} + \left(S\sum_{l = 0}^{n}\binom{n}{l}\vect z_0^{-l-1}\vect v_0^{(n-l)} + (D-\lambda)\sum_{l = 0}^{n}\binom{n}{l}\vect z_0^{-l}\vect v_0^{(n-l)} + E\sum_{l = 0}^{n}\binom{n}{l}\vect z_0^{-l+1}\vect z_0^{-l+1}\right)\right)
\end{align*}
Which yields the following condition for $\mathbf{u_i}$ to be an eigenvector
\begin{align*}
    \left(S + (D-\lambda_0)z_0 + Ez_0^2\right)\mathbf{v_1} &= - \left(S\sum_{l = 0}^{n}\binom{n}{l} \frac{j!}{(j-l)!}z_0^{-l}\vect v_0^{(n-l)} + (D-\lambda)\sum_{l = 0}^{n}\binom{n}{l} \frac{(j+1)!}{(j+1-l)!}z_0^{1-l}\vect v_0^{(n-l)}\right. \\
    &\qquad\qquad\qquad\qquad\qquad\qquad\left.+ E\sum_{l = 0}^{n}\binom{n}{l} \frac{(j+2)!}{(j+2-l)!}z_0^{2-l}\vect v_0^{(n-l)}\right)\\
    &= -\sum_{l = 0}^{n}\binom{n}{l} z_0^{-l}\left(S\frac{j!}{(j-l)!} z_0 + (D-\lambda)\frac{(j+1)!}{(j+1-l)!}z_0 + E\frac{(j+2)!}{(j+2-l)!} z_0^2\right) \mathbf{v_0}^{(n-l)}\\
    &= -\sum_{l = 0}^{n}\binom{n}{l} z_0^{-l} \frac{j!}{(j-l)!} \left(S+ (D-\lambda)(j+1)(j+1-l) z_0\right. \\
    &\qquad\qquad\qquad\qquad\qquad\qquad +\left. E (j+2)(j+2)(j+1-l)(j-l)z_0^2 \right)\mathbf{v_0}^{(n-l)}\\
    &= {\color{red} -\left( (D-\lambda) n \mathbf{w}^{(n-1)} + E(2nz_0\mathbf{w}^{(n-1)} + n(n-1)\mathbf{w}^{(n-2)} \right)}
\end{align*}\todo[color = red]{Show the red part is indeed true. Therefore use that $\mathbf{v_0}$ is an eigenvector to simplify terms.}


It remains to show that once we have obtained linearly independent eigenvectors\\ $(\mathbf{v_0})_1^{(p)}, \cdots, (\mathbf{v_0})_{n-p}^{(p)}$ that those are indeed eigenvectors to our problem therefore, we may use our previously derived condition.
First,  by (\ref{eq: confluent_n_roots}) may construct the $n-1$ first derivatives. \todo[color = yellow]{I will explain what $\mathbf{w}$ is and try not to abuse notation.}
\begin{itemize}
    \item For the term in $S$. We get by the chain rule
    \begin{equation}
        (\mathbf{w})^{(n)} = (\mathbf{w})^{(n)}
    \end{equation}
    \item For the term in $(D-\lambda)$ one gets by the chain rule:
    \begin{align*}
        (z_0\mathbf{w})^{(n)} &= \sum_{l = 0}^{n}\binom{n}{l}\vect (z_0)^{(l)}\vect w^{(n-l)}\\
        &= z_0 \mathbf{w}^{(n)} + n \mathbf{w}^{(n-1)}
    \end{align*}
    \item for the term in $E$ one gets
    \begin{align}
        (z_0^2\mathbf{w})^{(n)} &= \sum_{l = 0}^{n}\binom{n}{l}\vect (z_0^2)^{(l)}\vect w^{(n-l)}\\
        &= z_0^2 \mathbf{w}^{(n)} + 2nz_0\mathbf{w}^{n-1} + n(n-1)\mathbf{w}^{(n-2)}
    \end{align}
\end{itemize}

In other words (\ref{eq: confluent_n_roots}) yields:
\begin{equation}
   \left( S  + (D-\lambda) z_0  + E z_0^2 \right)(\mathbf{w})^{(n)}= - \left( (D-\lambda) n \mathbf{w}^{(n-1)} + E(2nz_0\mathbf{w}^{n-1} + n(n-1)\mathbf{w}^{(n-2)} \right) 
\end{equation}


Note that if they are all distinct we are done.
Assume that $n$, $1\leq n \leq m$ sequences $\mathbf{w_i}$ converge to the same $\mathbf{v_0}$. 

one can use those $n$ vectors $\mathbf{w_1},...,\mathbf{w_n}$ to construct an other vector. This vector can be constructed as follows. Let $\Delta(\epsilon_j) = z_{i}(\epsilon)-z_{i+1}(\epsilon_j)$
\begin{equation}
    \frac{\mathbf{w_1}(\epsilon_j)- \mathbf{w_2}(\epsilon_j)}{\Delta(\epsilon_j)} = (\mathbf{v_0})_1^{(1)}, \cdots, \frac{\mathbf{w_{n-1}}(\epsilon_j)- \mathbf{w_{n}}(\epsilon_j)}{\Delta(\epsilon_j)}= (\mathbf{v_0})_{n-1}^{(1)}
\end{equation}
where $(\mathbf{v_0})_i^{(1)}$ have been introduced for ease of notation.
(Note that this resembles the definition of a derivative. But since we are working in the complex plane, we can take the derivative along many paths. So this should be interpreted as a partial derivative along a path.) If those $(\mathbf{v_0})_i^{(1)}$ converge to different vectors, we are done, if some of them converge to the same vector we can again by the same process construct another vector of the form
\begin{equation}
    \frac{\frac{\mathbf{w_1}(\epsilon_j)- \mathbf{w_2}(\epsilon_j)}{\Delta(\epsilon_j)}-\frac{\mathbf{w_3}(\epsilon_j)- \mathbf{w_4}(\epsilon_j)}{\Delta(\epsilon_j)}}{\Delta(\epsilon_j)}=(\mathbf{v_0})_1^{(2)}, \cdots, \frac{\frac{\mathbf{w_{n-3}}(\epsilon_j)- \mathbf{w_{n-2}}(\epsilon_j)}{\Delta(\epsilon_j)}-\frac{\mathbf{w_{n-1}}(\epsilon_j)- \mathbf{w_n}(\epsilon_j)}{\Delta(\epsilon_j)}}{\Delta(\epsilon_j)}=(\mathbf{v_0})_{n-2}^{(2)} 
\end{equation}
If those obtained vectors $(\mathbf{v_0})_1^{(2)}, \cdots, (\mathbf{v_0})_{n-2}^{(2)}$ are again linearly dependent one could by a same procedure obtain vectors $(\mathbf{v_0})_1^{(p)}, \cdots, (\mathbf{v_0})_{n-p}^{(p)}$. By the same logic we consider
\begin{equation*}
    \frac{z_1\mathbf{w_1}(\epsilon_j)- z_2\mathbf{w_2}(\epsilon_j)}{\Delta(\epsilon_j)} = (z_0 \mathbf{v_0})_1^{(1)}
\end{equation*}
Using this simplified notation, we obtain by (\ref{eq: confluent_n_roots})
\begin{equation}
    S (z_0^0\mathbf{v_0})^{(n-1)} + (D-\lambda(\epsilon_j) + (z_0^1 \mathbf{v_0})^{(n-1)} + E (z_0^2 \mathbf{v_0})^{(n-1)} = 0
\end{equation}

If there exists a subsequence $\hat{\epsilon_j}$ of $\epsilon_j$ so that the norm of $(\mathbf{v_0})^{(p)}_{n-p}$ is bounded for $1 \leq p \leq n-1$, then we have shown existence of an eigenvector.
We show existence of such a subsequence $\hat{\epsilon_j}$ of $\epsilon_j$. Suppose therefore that no such sequence $\epsilon_j$ exists and that $(\mathbf{v_0})^{(p)}_{n-p}$ is unbounded for some $p$. 

As there exists a subsequence $\hat{\epsilon_j}$ such that $(\mathbf{v_0})^{(p)}_{n-p}$ tends to infinity.
This is 
\[
\babs{\frac{\Delta_{\vect w}(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}}\rightarrow +\infty, 
\]
which gives 
\begin{equation}
\babs{\frac{\Delta(\hat \epsilon_j)}{\Delta_{\vect w}(\hat \epsilon_j)}}\rightarrow 0. 
\end{equation}

{\color{blue} From here with the condition it should be straightforward to verify that the obtained vector is an eigenvector. It remains to show that the eigenvector is bounded, but the argument should be the same as in the previous Lemma.}
\textbf{Possible solution:} Consider the characteristic polynomial $\operatorname{det}(f(z)- \lambda)$. As we are interested in the eigenvalues, i.e. in  the roots $\lambda$ we will treat $\operatorname{det}(f(z)-\lambda)$ as a polynomial in $\lambda$ with parameter $z$.
\begin{equation}
    \operatorname{det}(f(z)-\lambda) = (a_1(z)- \lambda)(a_2(z)- \lambda)(a_3(z)- \lambda)\cdot...\cdot (a_k(z)-\lambda) = 0
\end{equation}
where $a_1(z),..., a_k(z)$ functions in $z$. Furthermore, by Lax we know that since the matrix $f(z)$ is differentiable that the its eigenvalues are continuous which implies that the functions $a_1(z), ... a_n(z)$ are continuous in $z$.
Then it is easy to see that the eigenvalues have multiplicity greater than one if and only if some of the paths parameterized by  $a_1(z)- \lambda = 0,..., a_k(z)- \lambda = 0$ intersect. Then there are three possibilities. Either the paths don't intersect, they intersect in certain points (as in the tridiagonal case), or they intersect on the entire path, e.g. $a_1(z) = a_2(z), \forall z$. To conclude, we have eigenvectors of multiplicity greater than one for at most algebraically many $\lambda$'s that lie on a path.

\todo[color = yellow]{I just use this for orientation. We can delete it later.}
In this section, we will analyze banded block Toeplitz operators and matrices. In the case of $l = 2$ we obtain
\begin{equation*}
    T = \begin{pmatrix}
        A_0 & A_1 & A_2 & 0 & \cdots &  0 \\
        A_{-1} & A_0& \ddots & \ddots & \ddots & \vdots\\
        A_{-2} & \ddots & \ddots & \ddots &\ddots &  0\\
        0 & \ddots & \ddots &\ddots & \ddots & A_2 \\
        \vdots &  \ddots& \ddots &\ddots  &A_0 & A_1\\
        0 & \cdots & 0 &A_{-2} & A_{-1} & A_0
    \end{pmatrix} = \begin{pmatrix}
    D & E & 0 & \dots & 0 \\
    S & D & \ddots  & \ddots & \vdots \\
    0 & \ddots & \ddots & \ddots & 0 \\
    \vdots & \ddots & \ddots & \ddots & E\\
    0 & \dots & 0 & S & D \\
\end{pmatrix}
\end{equation*}
where $ S = \begin{pmatrix}
    A_{-2} & A_{-1} \\
    0 & A_{-1}
\end{pmatrix}, D = \begin{pmatrix}
    A_0 & A_1 \\
    A_{-1} & A_0
\end{pmatrix}, E = \begin{pmatrix}
    A_2 & 0 \\
    A_1 & A_2
\end{pmatrix}$. By a similar process, any $l-$ banded block Toeplitz matrix can be brought under this form.


% l-banded block Toeplitz operators proof



By the previous arguments, it is not hard to see that, for all other $\lambda$'s in a small enough neighborhood of $\lambda_0$, the $\det(f(z)-\lambda)=0$ have $m$ different roots $z_1,..., z_m$. Now, considering a sequence $\lambda(\epsilon_j)$ convergence to $\lambda_0$, we have the corresponding roots $z_1(\epsilon_j),..., z_m(\epsilon_j)$ and the eigenvector $\vect w_1(\epsilon_j),...,  \vect w_m(\epsilon_j)$ with 
\begin{equation}\label{equ:proof_band_expoentialdecay}
\bnorm{\vect w_1(\epsilon_j)}_2 = \cdots=\bnorm{\vect w_m(\epsilon_j)}_2 =1,
\end{equation}
and 
\begin{align*}\label{equ:proof_band_expoentialdecay10}
&\vect w_1(\epsilon_j)\rightarrow \vect v_0\\
&\qquad\quad\vdots   \\
&\vect w_m(\epsilon_j) \rightarrow \vect v_m.
\end{align*}
possibly some vectors $\mathbf{v_i}$ may coincide. \todo[color = cyan]
{They could also be linearly dependent} Note that if they are all distinct we are done.
Assume that $n$, $1\leq n \leq m$ sequences $\mathbf{w_i}$ converge to the same $\mathbf{v_0}$.
Moreover, we have the following relation,
\begin{equation}\label{eq: confluent_n_roots}
\begin{cases}
\left(S+(D-\lambda(\epsilon_j))z_1(\epsilon_j)+Ez_1(\epsilon_j)^{2}\right) \vect {w_1}(\epsilon_j) =0,\\
\qquad\qquad\qquad\qquad\qquad\vdots\\
\left(S+(D-\lambda(\epsilon_j))z_n(\epsilon_j)+Ez_n(\epsilon_j)^{2}\right) \vect {w_n}(\epsilon_j) =0.
\end{cases}
\end{equation}
{\color{red} \textbf{Technicality 1:} We have to deal with the problem when we have that the vectors converge to a linear combination of previous vectors.}\\
{\color{blue}\textbf{Possible Solution:}
This technicality can be dealt with as follows. Suppose we have a $l$ linearly independent vectors $\vect a_i$ and that those $l$ vectors form a linear combination which we will call $\vect b$. We then have $l +1$ vectors but only $l$ are linearly independent.
\begin{equation*}
    \vect b = \sum_{i=1}^l c_i \vect a_i
\end{equation*}
Then one can recover another vector $\vect b_1$ by computing
\begin{equation}
    \frac{\vect b(\epsilon_j) - \sum_{i=1}^l c_i \vect a_i(\epsilon_j)}{\Delta(\epsilon_j)} 
\end{equation}
}
\todo[color = cyan]{It is not obvious how this works, since computing the "derivative" depends on $\Delta(\epsilon_j)$ and we have no canonical way of defining this here}
{\color{red}\textbf{Technicality 2:} It is possible that the sequences $\vect w_i$ converge to different vectors $\vect v_0$. In that case, there is no need to do the construction. However, It could also be that the constructed "derivatives" all converge to different vectors, or that some of them converge to the same vectors. In which case it would not be necessary to construct further derivatives.}\\
{\color{blue}
\textbf{Possible solution:} just say that we'll proceed in this manner until all the vectors are linearly independent and then we treat the "worst" case in the proof.}\\

{
%\color{blue}
We prove the statement by induction\\
\textbf{Basis:} Suppose that we have a double root $z_0$ and one corresponding eigenvector $\vect v_0$, then by Lemma\ref{lemma: double_root_technicality} we can construct a vector $\vect v_1$ such that 
\[
\mathbf{u_2} = (\mathbf{v_1}, z_0\mathbf{v_1}+\mathbf{v_0}, z_0^2\mathbf{v_1}+2z_0\mathbf{v_0}, \cdots).
\]
which is indeed of the correct form.\\
\textbf{Hypothesis:} Suppose that we have $n$ confluent roots, then we may recover $n-1$ vectors which are of the form
\begin{equation}
    (\vect v_0)^{(i)} \quad 1 \leq i \leq n-1
\end{equation}
and are bounded, i.e. we claim existence of a subsequence $\hat{\epsilon_j}$ of $\epsilon_j$ such that the norm of $\frac{\vect v_1^{(n-2)}(\epsilon_j) - \vect v_2^{(n-2)}(\epsilon_j)}{\Delta \epsilon_j}$ is bounded. Therefore, the $m$ eigenvectors take the form
\begin{equation*}
        \vect u_i = \left( \sum_{l = 0}^{i}\binom{i}{l}\vect v_0^{(i-l)},  \sum_{l = 0}^{i}\binom{i}{l}\vect (z_0)^{(l)}\vect v_0^{(i-l)},\sum_{l = 0}^{i}\binom{i}{l}\vect (z_0^2)^{(l)}\vect v_0^{(i-l)}, \cdots \right) \quad i  \in \{0,..., m-1\}
    \end{equation*}
\textbf{Step:} Suppose that we have $n+1$ confluent roots. We show that we may recover $n$ vectors. From the induction hypothesis, we know that for the first $n$ confluent roots we may recover $n-1$ vectors. First note that we get an additional relation of the form
\begin{equation*}
    \left(S+(D-\lambda(\epsilon_j))z_n(\epsilon_j)+Ez_n(\epsilon_j)^{2}\right) \vect {w_{n+1}}(\epsilon_j) =0
\end{equation*}
and by assumption $\vect {w_{n+1}} \to v_0$. Then one may construct a higher derivative 
\begin{equation}
    (\vect v_0)^{(n)}.
\end{equation}
This allows us to recover an additional eigenvector, such that we obtain a total of $n+1$ eigenvectors. We claim that those eigenvectors look as follows
\begin{equation*}
        \vect u_i = \left( \sum_{l = 0}^{i}\binom{i}{l}\vect v_0^{(i-l)},  \sum_{l = 0}^{i}\binom{i}{l}\vect (z_0)^{(l)}\vect v_0^{(i-l)},\sum_{l = 0}^{i}\binom{i}{l}\vect (z_0^2)^{(l)}\vect v_0^{(i-l)}, \cdots \right) \quad i  \in \{0,..., m\}
    \end{equation*}
By the induction hypothesis, we know that the vectors $\vect u_i$ for $i \in \{1,..., m-1\}$ are eigenvectors. But by construction of the derivatives using (\ref{eq: confluent_n_roots}) we know that
\begin{equation}
    \left( S + (D- \lambda) + E\right) \vect u_m = 0
\end{equation}
so that $\vect u_m$ is an eigenvector to the problem.
It remains to show that the $n$-th\todo[color = yellow]{This argument is still sloppy, it should also need the induction hypothesis.} derivative of the vector exists, i.e. that $(\vect v_0)^{(n)} $ is bounded. Therefore we show that there exists a subsequence $\hat{\epsilon_j}$ of $\epsilon_j$ such that the norm of $\frac{\vect v_1^{(n-1)}(\epsilon_j) - \vect v_2^{(n-1)}(\epsilon_j)}{\Delta \epsilon_j}$ is bounded. Note that by the Induction hypothesis that the expressions for $\vect v_1^{(n-1)}(\epsilon_j)$ and $\vect v_2^{(n-1)}(\epsilon_j)$ are well defined and in particular bounded. We argue by contradiction. Assume that there doesn't exists a subsequence $\hat{\epsilon_j}$ of $\epsilon_j$ such that the norm is bounded, i.e. $\frac{\vect v_1^{(n-1)}(\epsilon_j) - \vect v_2^{(n-1)}(\epsilon_j)}{\Delta \epsilon_j}$ tends to infinity. This is 
\[
\babs{\frac{\Delta_{\vect w}(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}}\rightarrow +\infty, 
\]
which gives 
\begin{equation}\label{eq: sequence to zero}
\babs{\frac{\Delta(\hat \epsilon_j)}{\Delta_{\vect w}(\hat \epsilon_j)}}\rightarrow 0. 
\end{equation}
Let $\Delta_{\vect w}(\epsilon_j) := \lVert \vect w_i (\epsilon_j) - \vect w_{i+1}(\epsilon_j) \rVert_2$, then let us again introduce some notation.
\begin{equation}
    \frac{\mathbf{w_1}(\epsilon_j)- \mathbf{w_2}(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)} = (\vect w / \Delta_{\vect w})^{(1)}_1, \cdots, \frac{\mathbf{w_{n-1}}(\epsilon_j)- \mathbf{w_{n}}(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}=(\vect w / \Delta_{\vect w})^{(1)}_{n-1}
\end{equation}
Using the same logic as we used previously, we obtain for the higher derivatives $(\vect w / \Delta_{\vect w})^{(n-1)}$.
also using (\ref{eq: confluent_n_roots})
\begin{equation}
    S (z_0^0\vect w / \Delta_{\vect w})^{(n-1)} + (D-\lambda(\epsilon_j) + (z_0^1 \vect w / \Delta_{\vect w})^{(n-1)} + E (z_0^2 \vect w / \Delta_{\vect w})^{(n-1)} = 0
\end{equation}
Note that by (\ref{eq: sequence to zero} indicates that there exists a subsequence $\Tilde{\epsilon_j}$ of $\hat{\epsilon_j}$ such that
\begin{equation}
    \lim_{\Tilde{\epsilon_j}\to 0}(S + (D-\lambda(\epsilon_j)z_0 + Ez_0^2)( \vect w/\Delta_{\vect w})^{(n-1)} = 0
\end{equation}
\todo[color=cyan]{I think we need to come up with a new argument for the boundedness. Here, we cannot just argue that there cant be another eigenvector since for general (non-tridiagonal) symbols, there might be many different ones}
\todo[color = yellow]{I agree!}
This concludes the proof of boundedness.
It remains to show that this new vector is orthogonal to the $n-1$ vectors obtained by the induction hypothesis. Therefore use that the new vector is the derivative of the previous vectors and hence lies in an orthogonal subspace of those vectors. So indeed this new vector is linearly independent to the previous vectors. This concludes the inductive proof.

}



\begin{lemma}
For the case, $v_1, v_1, v_2$.
\end{lemma}
\begin{proof}
\begin{align*}
&\vect w_1(\epsilon_j)\rightarrow \vect v_1\\
&\vect w_2(\epsilon_j)\rightarrow \vect v_1\\
&\vect w_3(\epsilon_j) \rightarrow \vect v_2.
\end{align*}
We define the space spanned by $\vect v_1, \vect v_2$ by $S_{1,2}$ and the projection $\mathcal P_{S_{1,2}}, \mathcal P_{S_{1,2}^{\perp}}$. Then consider 
\begin{equation}
\begin{aligned}
&S\frac{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}{\Delta_{p}(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_1(\epsilon_j)(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta_{p}(\epsilon_j)}+E \frac{z_1(\epsilon_j)^2(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta_{p}(\epsilon_j)}\\
=&- \left((D-\lambda(\epsilon_j))\frac{(z_1(\epsilon_j)-z_2(\epsilon_j))\vect w_2(\epsilon_j))}{\Delta_{p}(\epsilon_j)}+E \frac{(z_1(\epsilon_j)^2-z_2(\epsilon_j)^2)\vect w_2(\epsilon_j)}{\Delta_{p}(\epsilon_j)}\right)
\end{aligned}
\end{equation}
where 
\begin{align*}
&\Delta_1(\epsilon_j) = z_1(\epsilon_j) -z_2(\epsilon_j), \\
&\Delta_2(\epsilon_j) = \bnorm{\mathcal P_{S_{1,2}^{\perp}}(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}_2,\\
&\Delta_3(\epsilon_j) = \bnorm{\mathcal P_{S_{1,2}}(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}_2.
\end{align*}
If $\Delta_1(\epsilon_j)$ is of the largest order, then we are done. If $\Delta_{2}(\epsilon_j)$ is of the largest order, we are also done. If $O(\Delta_1(\epsilon_j))\ll (\text{or $\approx$}) O(\Delta_2(\epsilon_j))\ll O(\Delta_3(\epsilon_j))$. Then 
\begin{equation}
\begin{aligned}
&\left(S+(D-\lambda(\epsilon_j))z_1(\epsilon_j)+Ez_1(\epsilon_j)^2\right)\frac{\mathcal P_{S_{1,2}^{\perp}}(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta_{2}(\epsilon_j)}\\
&+ \left((D-\lambda(\epsilon_j))\frac{(z_1(\epsilon_j)-z_2(\epsilon_j))\vect w_2(\epsilon_j))}{\Delta_{2}(\epsilon_j)}+E \frac{(z_1(\epsilon_j)^2-z_2(\epsilon_j)^2)\vect w_2(\epsilon_j)}{\Delta_{2}(\epsilon_j)}\right)\\
=& \left(S+(D-\lambda(\epsilon_j))z_1(\epsilon_j)+Ez_1(\epsilon_j)^2\right)\frac{\mathcal P_{S_{1,2}}(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta_{2}(\epsilon_j)}.
\end{aligned}
\end{equation}
Note that the LHS convergences and thus the RHS convergences. 
\end{proof}

{\color{blue}\textbf{Different Approach:} For confluent roots $z_1, ..., z_m$ corresponding to $\lambda_0 $ we have that the vectors $\vect v_1, \vect v_2,...\vect v_m$ are not linearly independent anymore. By a previous argument , we know that for every $\lambda_0$ (for which roots $z_1, ..., z_m$ are confluent), there exists a neighbourhood, such that all the eigenvectors $\vect v_1, \vect v_2,...\vect v_m$ are linearly independent. Note that for those $m$ vectors to be linearly independent we must have that the vectorspace they belong to is at least $m$-dimensional. In particular any vector $\vect v_i$ is linearly independent to a subspace spanned by the other $(m-1)$ vectors.
Now as we take a sequence $\epsilon_j$, such that $\lambda \to \lambda_0$ the vectors $\vect v_i$ could become parallel or linearly dependent.
\begin{itemize}
    \item In the case where the vectors become \textbf{parallel}, we may do our derivative construction and by the previous argument we know that the derivative is orthogonal to the subspace, that means that the resulting derivative vector is orthogonal to all the other vectors.
    \item In the case where the vectors may become \textbf{linearly dependent}, proceed as follows. Suppose that $\vect v_1$ is a linear combination of $(m-1)$ vectors $\vect v_i$, i.e $\vect v_1 = \sum_{i=1}^{m-1} \alpha_i \vect v_i$. As we again do our derivative construction of $\vect w$, we have that this resulting derivative becomes orthogonal to the linear subspace $\{\vect v_2, \vect v_3,...,\vect v_m \}$.
\end{itemize}
\textbf{Very Important Remark: } If this construction is correct it would be sufficient to only take one derivative.\\

\noindent
\textbf{My intuitive understanding: }Suppose a vector becomes linearly dependent of other vectors, then the derivative points into the space where the vector came from.
}



\begin{lemma}\label{lemma: confluent_block_Toeplitz}
    Suppose $z_0$ is a root of multiplicity $m$ where $2\leq m \leq l$ for $\lambda_0$ and $\mathbf{v_0}$ is the only eigenvector corresponding to the eigenvalue $\lambda_0$ for $f(z_0)$ up to scaling, then prove that there exists a $\vect v_1, \cdots, \vect v_{m-1}$ that result from 
    \begin{equation}
        (z_0^j\mathbf{v_0})^{(n)} = \sum_{l = 0}^{n}\binom{n}{l}\vect (z_0^j)^{(l)}\underbrace{\vect v_0^{(n-l)}}_{\vect v_{n-l}}\mathds{1}_{j > l}
    \end{equation}
    such that,
    %\todo[color = yellow]{Still to be modified once we have the structure of the problem.}
    %\begin{equation*}
    %    \mathbf{u_i} = (\mathbf{v_1} + (z_0^0\mathbf{v_0})^{(i)}, z_0 \mathbf{v_1} + (z_0^1 \mathbf{v_0}){^{(i)}}, z_0^2\mathbf{v_1} + (z_0^2\mathbf{v_0})^{(i)}, ...) \quad i  \in \{1,..., m-1\}
    %\end{equation*}
    {
    \begin{equation*}
        \vect u_i = \left( \sum_{l = 0}^{i}\binom{i}{l}\vect v_0^{(i-l)},  \sum_{l = 0}^{i}\binom{i}{l}\vect (z_0)^{(l)}\vect v_0^{(i-l)},\sum_{l = 0}^{i}\binom{i}{l}\vect (z_0^2)^{(l)}\vect v_0^{(i-l)}, \cdots \right) \quad i  \in \{0,..., m-1\}
    \end{equation*}
    }
    %\todo[color = yellow]{We should also be able to get rid of the binomial coefficients since we are dealing with vectors. However, I chose to keep them since it is easier to see them in the proof...}

    {\color{red} Motivation for the structure. From the Leibniz rule, one obtains
    \begin{itemize}
        \item First derivative: $(\mathbf{v_0} z_0^j)' = \underbrace{\mathbf{v_0}'}_{= \vect v_1}z_0^j + \mathbf{v_0} (z_0^j)' $. 
        \item Second derivative: $(\mathbf{v_0}z_0^j)'' = \underbrace{\mathbf{v_0}''}_{\vect v_2}z_0^j + 2\underbrace{\mathbf{v_0}'}_{\vect v_1}(z_0^j)' + \mathbf{v_0}(z_0^j)''$.
        \item $n$-th derivative:
        $(z_0^j\mathbf{v_0})^{(n)} = \sum_{l = 0}^{n}\binom{n}{l}\vect (z_0^j)^{(l)}\underbrace{\vect v_0^{(n-l)}}_{\vect v_{n-l}}\mathds{1}_{j > l}$
    \end{itemize}
    }
\end{lemma}


% \section{Spectra and pseudo-spectra  of l-banded Block-Toeplitz operators and matrices}
% In this section we will characterize the spectrum of $l$-banded block-Toeplitz operators and present a similar result as in the case with tridiagonal Toeplitz operators.
% \subsection{Spectra of l-banded Block-Toeplitz operators}

% First we recall the definition of such a class of operators.
% \begin{definition}
%     We say that an operator is $l$-banded block-Toeplitz if it's associated semi-infinite matrix is $l$-banded and its entries $(a_n)_{n \in \mathbb{N}}$ are sequences of $N\times N$ matrices.
% \end{definition}

% In the case of block Toeplitz operators, it is much more difficult to fully characterize the spectrum, to see why consider the following example found in \cite[Example 6.1]{bottcher.silbermann1999Introduction}


% Despite these complications, we managed to fully characterize the spectrum of banded block Toeplitz operators. To the best of our knowledge, this is the first such result for banded block Toeplitz operators. This was done by using constructions employed by Trefethen in his proof of \cite{REICHEL1992153} as well as some non-trivial observations about $\det(f(z)-\lambda)$.

% \begin{theorem}
%     Let $f \in \mathbf{C}^{k\times k}$ be the symbol of a tri-block Toeplitz operator $T(f)$. The spectrum $\sigma(T(f))$ of $T(f)$ is given by the following
%     \begin{align*}
%         \sigma(T(f)) &= \sigma_P(f(\mathbb{T})) \cup \{\lambda \in \C\setminus \sigma_P(f(\mathbb{T})):\operatorname{wind}(\det(f-\lambda),0)\neq 0\}\\
%         &\cup \{\lambda \in \C\setminus \sigma_P(f(\mathbb{T})):  \operatorname{wind}(\det(f-\lambda),0)\text{ and }\\
%         &\operatorname{Span}(\cup_{z\in D:\det(f(z)-\lambda)=0}\operatorname{Eig}(\lambda,f(z)))\cap \ker(A_{-1})\neq \vect 0\}.
%     \end{align*}
% \end{theorem}



% %\begin{theorem}
% %Exponentially decay or increasing.
% %\end{theorem}
% \subsection{Pseudo-spectra  of l-banded Block Toeplitz operators and matrices}
% Now that we have established a general framework on tridiagonal Toeplitz matrices, we can extend Theorem\ref{thm: exponential_decay_k_operators} to a more general framework, namely to $l$-banded Block Topelitz matrices. \\
% \begin{theorem}[Exponential decay of l-Banded block Toeplitz operators]\label{thm: exponential_decay_Block_operators}
% Let $\{\mathbf{A}_N \}$ be a family of $l$-banded block Toeplitz operators and let $\lambda$ be any complex number such that $\operatorname{wind}(\operatorname{det}(f(z)-\lambda) <0$. Then for some $\rho < 1$ and all sufficiently large $N$,
% \begin{equation}
%         \lVert (\lambda-\mathbf{A}_N)^{-1}\rVert \geq \rho^{N},
%     \end{equation}
%     there exist \emph{almost surely} non-zero pseudo-eigenvectors \(\mathbf{v}_{(N)}\) satisfying
%     \begin{equation}
%         \frac{\lVert (\mathbf{A}_N-\lambda)\mathbf{v}^{(N)}\rVert}{\lVert \mathbf{v}^{(N)}\rVert} \leq \rho^{N}
%     \end{equation}
%     such that 
% \end{theorem}
% \begin{proof}
% Now we prove the existence of such that the set of $\lambda$'s for which we have confluent roots has measure zero.
% Let $\operatorname{det}(f(z)-\lambda)$ be a polynomial of degree $n$ in $z$ with coefficients $a_i(\lambda)$ that are polynomials in $\lambda$:
% \begin{equation*}
%     \operatorname{det}(f(z)-\lambda) = a_n(\lambda)z^n + a_{n-1}(\lambda)z^{n-1} + \ldots + a_1(\lambda)z + a_0(\lambda)
% \end{equation*}
% The polynomial $\operatorname{det}(f(z)- \lambda)$ has roots of multiplicity greater than one if and only if its discriminant is equal to 0 as a function of $\lambda$, i.e. $\Delta(\lambda) =0$.
% The discriminant of $\operatorname{det}(f(z)-\lambda)$ is defined as:
% \begin{equation}
%     \Delta(\lambda) = \prod_{i < j} (z_i(\lambda) - z_j(\lambda))^2
% \end{equation}
% where $z_i(\lambda)$ are the roots of $\operatorname{det}(f(z)-\lambda)$. 
% The set of $\lambda$'s that satisfy $\Delta(\lambda) = 0$ is a submanifold of $\C$ and thus has to be either a curve or a set of discrete points. In particular, it has measure zero in $\C$.
% \end{proof}

% Note that Theorem\ref{thm: exponential_decay_Block_operators} only gives us that almost surely there exists an exponentially decaying pseudoeigenvector. If we restrict Theorem\ref{thm: exponential_decay_Block_operators} to matrices get a stronger result.

% \begin{theorem}[Exponential decay of l-Banded block Toeplitz matrices]\label{thm: exponential_decay_Block_matrices}
    
% \end{theorem}


% We now address the case where some of the roots $z_1,..., z_l$ are confluent. It is enough to consider the case where the root $z_0$ has multiplicity at most $l$. 
% %First note that the $n$-th derivative of the monomial $z^j$ is given by 
% %    \begin{equation*}
% %        (z^j)^{(n)} = \begin{cases}
% %           j \cdot (j-1)\cdot...\cdot (j-n+1) z^{j-n} & j\geq n\\
% %           0 & j < n
% %        \end{cases}
% %    \end{equation*}
% %Also note that alternatively one can define the $n$-th derivative of a function as
% %\begin{equation}
% %    g(z)^{(n)} = \lim_{\epsilon \to 0} \frac{g(z + \epsilon)^{(n-1)}- g(z)^{(n-1)}}{\epsilon}
% %\end{equation}



% \begin{theorem}\label{thm: exponential decay, stronger version}
%     Let \(\{\mathbf{A}_N\}\) be a family of l-diagonal, k-Toeplitz operators and let \(\lambda\) be any complex number with \(\operatorname{wind}(\det(f-\lambda),0) \neq 0\). Then for some \(M>1\) and all sufficiently large N ,
%     \begin{equation}
%         \lVert (\lambda-\mathbf{A}_N)^{-1}\rVert \geq M^{-N},
%     \end{equation}
%     and there exist non-zero pseudoeigenvectors \(\mathbf{v}_{(N)}\) satisfying
%     \begin{equation}
%         \frac{\lVert (\mathbf{A}_N-\lambda)\mathbf{v}^{(N)}\rVert}{\lVert \mathbf{v}^{(N)}\rVert} \leq M^{-N}
%     \end{equation}
%     such that 
%     \begin{equation}
%         \frac{|v_j^{(N)}|}{\max|v_j^{(N)}|} \leq
%         \begin{cases}
%             M^{-j} & \text{if } \operatorname{wind}(\det(f-\lambda),0) < 0, \\
%             M^{j-N} & \text{if } \operatorname{wind}(\det(f-\lambda),0) > 0,
%         \end{cases}
%         \quad 1\leq j \leq N.
%     \end{equation}
% \end{theorem}





% %\todo{NEEDS CHECKING} 
% \begin{proof}
%     Let \(\lambda \in \mathbf{C}\) such that \(\operatorname{wind}(\det(f-\lambda),0)<0\). Observe that \(\det(f-\lambda)\) is a meromorphic function in the unit disk with \(\frac{l-1}{2}\) poles at 0. By the argument principle, this implies that \(\det(f-\lambda) = 0\) for  \(\frac{l-1}{2} + 1\) values \(z_i\). Assume for simplicity that these values are distinct. This implies that \(\lambda\) is an eigenvalue of \(f(z_i)\), let \(v_i\) denote an associated eigenvector. Consider the vectors defined by
%     \begin{equation}
%         \mathbf{u}_i= (\mathbf{v}_i, z_i \mathbf{v}_i, z_i^2 \mathbf{v}_i, \dots)^\top.
%     \end{equation}
%     They satisfy the eigenvalue equation \(\mathbf{A}_N \mathbf{u}_i = \lambda u_i\) in the rows \(j \geq \frac{l-1}{2}\). For a linear combination \(\mathbf{u}\) of the vectors \(\mathbf{u}_i\) to be an eigenvector, it is a necessary and sufficient condition that \(\mathbf{u}\) satisfies the eigenvalue problem in the rows \(1 \leq j \leq \frac{l-1}{2}\). This is a linear system of \(\frac{l-1}{2}\) equations, since we have \(\frac{l-1}{2}+1\) linear independent vectors \(\mathbf{u}_i\), a unique solution exists. 

%     %TODO: Are the \(z_i\) always distinct? @Ping: does your proof for the confluent Vandermonde matrix work here?

%     This completes the proof under the assumption that the roots $z_1, \ldots, z_l$ are distinct. If some of the roots $z_0, \ldots, z_l$ are confluent at some points $\lambda \in \bar{\Omega}_r$ we apply Lemma\ref{lemma: confluent_block_Toeplitz}.
% \end{proof}


%\subsection{Numerical illustration}



The polynomial $\operatorname{det}(f(z)- \lambda)$ has roots of multiplicity greater than one if and only if its discriminant is equal to 0 as a function of $\lambda$, i.e. $\Delta(\lambda) =0$.
The discriminant of $\operatorname{det}(f(z)-\lambda)$ is defined as:
\begin{equation}
    \Delta(\lambda) = \prod_{i < j} (z_i(\lambda) - z_j(\lambda))^2
\end{equation}
{\color{red} This doesn't work suppose $p(\lambda, z) = (z - \lambda)^2$ , such that $z_1(\lambda) = z_2(\lambda) = \lambda$ then $\Delta(\lambda) = 0, \quad \forall \lambda \in \C$ and doesn't have measure zero. without much information about the polynomial we can't deduce a result of the kind, for all polynomials the set of $\lambda$'s for which we have roots with multiplicity greater than one has measure 0.}
where $z_i(\lambda)$ are the roots of $\operatorname{det}(f(z)-\lambda)$. Moreover, it is a well-known result that the roots of a polynomial depend continuously on the coefficients of the polynomial, such that the $z_1(\lambda)$ are continuous in lambda. As a direct consequence $\Delta(\lambda)$ is also continuous in $\lambda$ as the composition of continuous functions. Note that the roots $z_i(\lambda)$ are isolated (even if the root has a multiplicity greater than one. Isolated roots mean just that in a neighborhood of the root, there are no more distinct roots). In particular then also the roots of $\Delta(\lambda)$ are isolated.
The set of $\lambda$'s that satisfy $\Delta(\lambda) = 0$ is a submanifold\todo[color=cyan]{Why? elaborate}
\todo[color = yellow]{I think the Diffgeo argument is a bit overkill, We should just use the fact that a line in $\R^2$ has measure 0. }
\todo[color = yellow]{We could do a numerical visualization. What do you think?}of $\C$ and thus has to be either a curve or a set of discrete points. In particular, it has measure zero in $\C$. This concludes the proof.



% \todo{Check the paper in the group, and write down as much as possible results and discussions. }
% \begin{theorem}\label{thm: exponential_decay_k_operators}
% Let \(\{\mathbf{A}_N\}\) be a family of tridiagonal $k$-Toeplitz operators and let \(\lambda\) be any complex number with \(\operatorname{wind}(\det(f(z)-\lambda),0) < 0\). Then for some \(\rho <1\) and all sufficiently large N , \todo{write $\rho<1$ instead of $M>1$.}
%     \begin{equation}
%         \lVert (\lambda-\mathbf{A}_N)^{-1}\rVert \geq \rho^{N},
%     \end{equation}
%     and there exist non-zero pseudo-eigenvectors \(\mathbf{v}_{(N)}\) satisfying
%     \begin{equation}
%         \frac{\lVert (\mathbf{A}_N-\lambda)\mathbf{v}^{(N)}\rVert}{\lVert \mathbf{v}^{(N)}\rVert} \leq \rho^{N}
%     \end{equation}
%     such that 
%     \begin{equation}\label{bound l =1}
%         \frac{|v_j^{(N)}|}{\max|v_j^{(N)}|} \leq
%         \begin{cases}
%             \rho^{j} & \text{if } \operatorname{wind}(\det(f-\lambda),0) < 0, \\
%             \rho^{N-j} & \text{if } \operatorname{wind}(\det(f-\lambda),0) > 0,
%         \end{cases}
%         \quad 1\leq j \leq N.
%     \end{equation}
% \end{theorem}

% \begin{proof}
%     Let \(\lambda \in \mathbf{C}\) such that \(\operatorname{wind}(\det(f-\lambda),0)<0\). Observe that \(\det(f-\lambda)\) is a meromorphic function in the unit disk, with a pole at 0. By the argument principle, this implies that \(\det(f-\lambda) = 0\) for two values \(z_1,z_2\), counted with multiplicity. Moreover, since \(\det(f(z_i)-\lambda) = 0\), we find that \(\lambda \) is an eigenvalue to \(f(z_i)\) and hence there exists an associated eigenvector \(\mathbf{v}_i\). Assume for now that \(z_1 \neq z_2\) and as well as that the associated eigenvectors are distinct.\todo[color = yellow]{Maybe write that the vectors are linearly independent.} Consider now the vectors defined by
%     \begin{equation}
%         \mathbf{u}_i= (\mathbf{v}_i, z_i \mathbf{v}_i, z_i^2 \mathbf{v}_i, \dots)^\top \quad i \in \{1,2\}.
%     \end{equation}
%     This vector satisfies the eigenvalue equation \(\mathbf{A}_N\mathbf{u}_i = \lambda\mathbf{u}_i\) in all but the first row. Since $u_1, u_2$ are linearly independent, there exists a linear combination of them that is indeed an eigenvector of \(\mathbf{A}\).

   
%     By Lemma\ref{lemma: double_root_technicality} we may conclude the existence of eigenvectors in the case where the roots are confluent. Therefore, one can always find two linearly independent vectors to construct the pseudo-eigenvector.


%     %\textbf{Current Idea:}Construct Cauchy sequence of $u_i$. 
% \end{proof}

% The technicality with confluent roots in the proof of Theorem\ref{thm: exponential_decay_k_operators} can be dealt with as follows. But first note the following

% \begin{lemma}\label{lemma: double_root_technicality}
% Suppose $z_0$ is the double root for $\lambda_0$ and $\mathbf{v_0}$ is the only eigenvector corresponding to eigenvalue $\lambda_0$ for $f(z_0)$ up to a scaling, then prove that there exists $\mathbf{v_1}$ so that the 
% \[
% \mathbf{u_2} = (\mathbf{v_1}, z_0\mathbf{v_1}+\mathbf{v_0}, z_0^2\mathbf{v_1}+2z_0\mathbf{v_0}, \cdots).
% \]
% \end{lemma}
% \begin{proof}
% For $\mathbf{u_2}$ to be an eigenvector, for $j\geq 1$ we find the condition
% \begin{align*}
% &S(z_0^j\mathbf{v_1}+jz_0^{j-1}\mathbf{v_0})+(D-\lambda_0)(z_0^{j+1}\mathbf{v_1}+(j+1)z_0^{j}\mathbf{v_0})+E(z_0^{j+2}\mathbf{v_1}+(j+2)z_0^{j+1}\mathbf{v_0})\\
% =&z_0^{j}\left(S(\mathbf{v_1}+jz_0^{-1}\mathbf{v_0})+(D-\lambda_0)(z_0\mathbf{v_1}+(j+1)\mathbf{v_0})+E(z_0^{2}\mathbf{v_1}+(j+2)z_0\mathbf{v_0})\right)\\
% =& z_0^{j}\left(S(\mathbf{v_1})+(D-\lambda_0)(z_0\mathbf{v_1}+\mathbf{v_0})+E(z_0^{2}\mathbf{v_1}+2z_0\mathbf{v_0})\right)
% \end{align*}
% Thus we only need 
% \begin{equation}
% \left(S+(D-\lambda_0)z_0+Ez_0^{2}\right) \mathbf{v_1} = -\left((D-\lambda_0)+2Ez_0\right) \mathbf{v_0}.
% \end{equation}
% Now we prove the existence of such $\vect v_1$ in the case where the roots $z_1$ and $z_2$ are confluent. By the previous arguments, it is not hard to see that, for all other $\lambda$'s in a small enough neighborhood of $\lambda_0$, the $\det(f(z)-\lambda)=0$ have two different roots $z_1, z_2$. Note that by Remark\ref{rem: discrete_lambdas_tridiagonal} we know that the $\lambda$'s are discrete points such that a neighborhood of $\lambda_0$ exists. Now, considering a sequence $\lambda(\epsilon_j)$ convergence to $\lambda_0$, we have the corresponding roots $z_1(\epsilon_j), z_2(\epsilon_j)$ and the eigenvector $\vect w_1(\epsilon_j), \vect w_2(\epsilon_j)$ with 
% \begin{equation}\label{equ:proofexpoentialdecay9}
% \bnorm{\vect w_1(\epsilon_j)}_2 = \bnorm{\vect w_2(\epsilon_j)}_2 =1,
% \end{equation}
% and 
% \begin{equation}\label{equ:proofexpoentialdecay10}
% \vect w_1(\epsilon_j)\rightarrow \vect v_0,\quad  \vect w_2(\epsilon_j) \rightarrow \vect v_0.
% \end{equation}
% { As it is finite-dimensional and bounded, for unit $\vect w_1(\epsilon_j)$ so that 
% \[
% \left(S+(D-\lambda(\epsilon_j))z_1(\epsilon_j)+Ez_1(\epsilon_j)^{2}\right) \vect {w}_1(\epsilon_j) =\vect 0,
% \]
% there is a subsequence $\hat \epsilon_j$ so that $\lim_{\hat \epsilon_j\rightarrow 0} \vect {w}_1(\epsilon_j)$ exists and 
% \[
% \lim_{\hat \epsilon_j\rightarrow 0} \left(S+(D-\lambda(\hat \epsilon_j))z_1(\hat \epsilon_j)+Ez_1(\hat \epsilon_j)^{2}\right)\lim_{\hat \epsilon_j\rightarrow 0} \vect {w}_1(\hat \epsilon_j) =\vect 0.
% \]
% So 
% \[
% \vect w_1(\epsilon_j) \rightarrow \vect v_0
% \]
% and so dose $\vect w_2(\epsilon_j)$. 
% }

% %\todo[color=cyan]{Why can we simply pick these $w_i(\epsilon_j)$? If the eigenspace of $f(z(\epsilon_j))$ associated to $\lambda(\epsilon_j)$ is not one-dimensional, there could be multiple linearly independent vectors, why should all of them tend to $v_0$?}
% %\todo[color=cyan]{After some more consideration, this might be fixable using a compactness argument that any sequence of $w_1(\epsilon_j$ must have a convergent subsequence and the only element it can converge to is $v_0$}
% %\todo{Right, this is why I confine the eigenspace to be one-dimensional and transform the problem to be finite-dimensional by considering only $S, D, E,$ rather than the Toeplitz operator $T$. The compact property is very important. }

% Since $\vect v_0$ is the only eigenvector of $f(z_0)$ corresponding to $\lambda_0$, the above properties can hold. In particular, we have 
% \begin{align*}
% &\left(S+(D-\lambda(\epsilon_j))z_1(\epsilon_j)+Ez_1(\epsilon_j)^{2}\right) \vect {w_1}(\epsilon_j) =0,\\
% &\left(S+(D-\lambda(\epsilon_j))z_2(\epsilon_j)+Ez_2(\epsilon_j)^{2}\right) \vect {w_2}(\epsilon_j) =0.\\
% \end{align*}
% It yields
% \begin{equation}\label{equ:proofexpoentialdecay4}
% \begin{aligned}
% &S\frac{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}{\Delta(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_1(\epsilon_j)\vect w_1(\epsilon_j)-z_2(\epsilon_j)\vect w_2(\epsilon_j)}{\Delta(\epsilon_j)}\\
% & \qquad +E\frac{z_1(\epsilon_j)^2\vect w_1(\epsilon_j)-z_2(\epsilon_j)^2\vect w_2(\epsilon_j)}{\Delta(\epsilon_j)} =0
% \end{aligned}
% \end{equation}
% where $\Delta(\epsilon_j):=z_1(\epsilon_j)-z_2(\epsilon_j)$ and 
% \begin{equation}\label{equ:proofexpoentialdecay5}
% \begin{aligned}
% &S\frac{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_1(\epsilon_j)\vect w_1(\epsilon_j)-z_2(\epsilon_j)\vect w_2(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}\\
% & \qquad +E\frac{z_1(\epsilon_j)^2\vect w_1(\epsilon_j)-z_2(\epsilon_j)^2\vect w_2(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)} =0
% \end{aligned}
% \end{equation}
% where $\Delta_{\vect w}(\epsilon_j):= \bnorm{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}_2$. Note that (\ref{equ:proofexpoentialdecay4}) gives 
% \begin{equation}\label{equ:proofexpoentialdecay3}
% \begin{aligned}
% &S\frac{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}{\Delta(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_1(\epsilon_j)(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta(\epsilon_j)}+E \frac{z_1(\epsilon_j)^2(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta(\epsilon_j)}\\
% =&- \left((D-\lambda(\epsilon_j))\frac{(z_1(\epsilon_j)-z_2(\epsilon_j))\vect w_2(\epsilon_j))}{\Delta(\epsilon_j)}+E \frac{(z_1(\epsilon_j)^2-z_2(\epsilon_j)^2)\vect w_2(\epsilon_j)}{\Delta(\epsilon_j)}\right).
% \end{aligned}
% \end{equation}
% If there exists a subsequence $\hat \epsilon_j$'s of $\epsilon_j$'s so that the norm of $\frac{\vect w_1(\hat \epsilon_j)-\vect w_2(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}$ is bounded, considering a subsequence of $\hat \epsilon_j$'s is enough to prove the existence of the limit and hence prove the existence of such $\vect v_1$ so that 
% \begin{equation}\label{equ:proofexpoentialdecay13}
% \left(S+(D-\lambda_0)z_0+Ez_0^{2}\right) \mathbf{v_1} = -\left((D-\lambda_0)+2z_0E\right) \mathbf{v_0}.
% \end{equation}
% Suppose now that there is no subsequence $\hat \epsilon_j$'s of $\epsilon_j$'s so that the norm of $\frac{\vect w_1(\hat \epsilon_j)-\vect w_2(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}$ is bounded. Thus there exists a subsequence $\hat \epsilon_j$'s of $\epsilon_j$'s so that the norm of $\frac{\vect w_1(\hat \epsilon_j)-\vect w_2(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}$ tends to infinity. This is 
% \[
% \babs{\frac{\Delta_{\vect w}(\hat \epsilon_j)}{\Delta(\hat \epsilon_j)}}\rightarrow +\infty, 
% \]
% which gives 
% \begin{equation}\label{equ:proofexpoentialdecay8}
% \babs{\frac{\Delta(\hat \epsilon_j)}{\Delta_{\vect w}(\hat \epsilon_j)}}\rightarrow 0. 
% \end{equation}
% On the other hand, (\ref{equ:proofexpoentialdecay5}) gives
% \begin{equation}\label{equ:proofexpoentialdecay7}
% \begin{aligned}
% &S\frac{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}+ (D-\lambda(\epsilon_j))\frac{z_1(\epsilon_j)(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta_{\vect w}(\epsilon_j)}+E \frac{z_1(\epsilon_j)^2(\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j))}{\Delta_{\vect w}(\epsilon_j)}\\
% =&- \left((D-\lambda(\epsilon_j))\frac{(z_1(\epsilon_j)-z_2(\epsilon_j))\vect w_2(\epsilon_j))}{\Delta_{\vect w}(\epsilon_j)}+E \frac{(z_1(\epsilon_j)^2-z_2(\epsilon_j)^2)\vect w_2(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}\right).
% \end{aligned}
% \end{equation}
% Then (\ref{equ:proofexpoentialdecay8}) indicates that there exists a subsequence $\tilde \epsilon_j$'s of $\hat \epsilon_j$'s so that 
% \[
% \lim_{\tilde \epsilon_j\rightarrow 0} (S+(D-\lambda(\tilde \epsilon_j))z_0 + 2z_0^2E)\frac{\vect w_1(\tilde\epsilon_j)-\vect w_2(\tilde\epsilon_j)}{\Delta_{\vect w}(\tilde\epsilon_j)} = \vect 0.
% \]
% Note that the boundedness of $\frac{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}{\Delta_{\vect w}(\epsilon_j)}$ is also important for deriving the above limit. This gives 
% \begin{equation}\label{equ:proofexpoentialdecay12}
% (S+(D-\lambda_0)z_0 + z_0^2E)\vect v_1 = \vect 0,
% \end{equation}
% for a certain vector $\vect v_1$ with $\bnorm{\vect v_1}_2=1$. Now we prove that $\vect v_1\neq \vect v_0$ and $\vect v_1 \neq -\vect v_0$. As $\vect v_1$ is the limit of 
% \[
% \frac{\vect w_1(\tilde\epsilon_j)-\vect w_2(\tilde\epsilon_j)}{\Delta_{\vect w}(\tilde\epsilon_j)},
% \]
% a key observation is that, since (\ref{equ:proofexpoentialdecay9}) and (\ref{equ:proofexpoentialdecay10}), the angle between 
% $\vect w_1(\tilde\epsilon_j)-\vect w_2(\tilde\epsilon_j)$ and $\vect v_0$ should approximate $\frac{\pi}{2}$. This is enough to demonstrate $\vect v_1\neq \vect v_0$ and $\vect v_1 \neq -\vect v_0$. Now, (\ref{equ:proofexpoentialdecay12}) contradicts the condition that $\vect v_0$ is the only eigenvector of $f(z_0)$ corresponding to the eigenvalue $\lambda_0$. Thus this case does not hold, we only have the case that $\frac{\vect w_1(\epsilon_j)-\vect w_2(\epsilon_j)}{\Delta(\epsilon_j)}$ are uniformly bound. Then (\ref{equ:proofexpoentialdecay13}) already demonstrates the existence. This completes the proof. 
%\end{proof}


\begin{remark}
     In the case of tridiagonal $k$-Toeplitz operators, using \ref{lem:tridiagonaldeterminant}
     we get an explicit formula for the winding of the symbol
    \begin{equation}
        \operatorname{wind}(\det(f - \lambda),0) = \frac{1}{2\pi}\int_0^{2\pi} \frac{(-1)^{k}(\prod_{i=1}^kc_i) e^{-i \theta} + (-1)^{k+1}(\prod_{i=1}^k b_i)e^{i \theta}}{(-1)^{k+1}(\prod_{i=1}^kc_i) e^{-i\theta} + (-1)^{k+1}(\prod_{i=1}^kb_i)e^{i\theta} + g(\lambda)}d\theta
    \end{equation}
    Note that this formula is useful to numerically compute the $\lambda$'s for which the winding number is non-trivial. Particularly, the spectrum as in Theorem \ref{thm:windingspectrum} may be simplified.
\end{remark}


==> preamble.tex <==

\usepackage{graphicx} 
\usepackage{amssymb, amsmath}
\usepackage{geometry}
\usepackage{minted}
\usepackage{hyperref}             
\usepackage{subfig}
\numberwithin{equation}{section} 
\usepackage{mdframed}
\usepackage[table]{xcolor}
\usepackage[backend=biber,style=alphabetic]{biblatex}
\addbibresource{bibliography.bib}         
\renewcommand{\baselinestretch}{1.04}        %line spacing
%\usepackage{afterpage}                      %emptypage
\usepackage[export]{adjustbox}

\hypersetup{
pdftitle={PROPERTIES OF $k-$TOEPLITZ MATRICES},
pdfsubject={Mathematics, Quantum Algebra, Q-calculus, Time-scale calculus},
pdfauthor={HABIB AMMARI, SILVIO BARANDUN, YANNICK DE BRUIJN,PING LIU, and CLEMENS THALHAMMER},
pdfkeywords={}
}

\newmdtheoremenv[backgroundcolor=green!0!white,linewidth=0pt,]{definition}{Definition}[section]
\newmdtheoremenv[backgroundcolor=yellow!0!white, linewidth=0pt,]{remark}{Remark}[section]
\newmdtheoremenv[backgroundcolor=yellow!0!white, linewidth=0.5pt,]{corollary}{Corollary}[section]
\newmdtheoremenv[backgroundcolor=red!0!white, linewidth=0.5pt,]{theorem}{Theorem}[section]
\newmdtheoremenv[backgroundcolor=red!0!white, linewidth=0.5pt,]{lemma}{Lemma}[section]
\newmdtheoremenv[backgroundcolor=white, linewidth=0pt,]{example}{Example}[section]

\newgeometry{inner = 3.5cm, outer = 3.5cm, top = 3.5cm, bottom = 3.5cm}
